Generative 3D Part Assembly via Part-Whole-Hierarchy Message Passing

Generative 3D part assembly involves understanding part relationships and predicting their 6-DoF poses for assembling a realistic 3D shape. Prior work often focus on the geometry of individual parts, neglecting part-whole hierarchies of objects. Leveraging two key observations: 1) super-part poses provide strong hints about part poses, and 2) predicting super-part poses is easier due to fewer superparts, we propose a part-whole-hierarchy message passing network for efficient 3D part assembly. We first introduce super-parts by grouping geometrically similar parts without any semantic labels. Then we employ a part-whole hierarchical encoder, wherein a super-part encoder predicts latent super-part poses based on input parts. Subsequently, we transform the point cloud using the latent poses, feeding it to the part encoder for aggregating super-part information and reasoning about part relationships to predict all part poses. In training, only ground-truth part poses are required. During inference, the predicted latent poses of super-parts enhance interpretability. Experimental results on the PartNet dataset show that our method achieves state-of-the-art performance in part and connectivity accuracy and enables an interpretable hierarchical part assembly. Code is available at https://github.com/pkudba/3DHPA.

==> tables/ablationdepth.tex <==
\begin{table}  
  \centering
  \caption{Ablation study on the depth of the part encoder.}
  \resizebox{0.65\columnwidth}{!}{%
  \begin{tabular}{lc|ccc}
    \toprule
    & layers &  SCD$\downarrow$ & PA$\uparrow$ & CA$\uparrow$ \\
    \midrule
    & 2 & 0.0044 & 56.32 & 40.86 \\
    \midrule
    & 4 & 0.0035 & 61.28 & 55.67 \\
    \midrule
    & 6 & \textbf{0.0028}  & \textbf{64.83} & \textbf{58.45} \\
    \midrule
    & 8 & 0.0030 & 63.26 & 57.39 \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:ablationdepth}  
\end{table}

==> tables/ablationsuperpartdepth.tex <==
\begin{table}
  \centering
  \caption{Ablation study on the depth of the super-part encoder.}
  \resizebox{0.65\columnwidth}{!}{%
  \begin{tabular}{lc|ccc}
    \toprule
    & layers &  SCD$\downarrow$ & PA$\uparrow$ & CA$\uparrow$ \\
    \midrule
    & 2 & \textbf{0.0028}  & \textbf{64.83} & \textbf{58.45} \\
    \midrule
    & 4 & 0.0029 & 63.49 & 57.62\\
    \midrule
    & 6 & 0.0031 & 63.00 & 56.93 \\
    \midrule
    & 8 & 0.0034 & 62.12 & 55.82 \\
    \bottomrule
  \end{tabular}
  }
  \label{tab:ablationsuperpartdepth}  
\end{table}
